Static and Dynamic Robust PCA and Matrix Completion: A Review

Principal Components Analysis (PCA) is one of the most widely used dimension reduction techniques. Robust PCA (RPCA) refers to the problem of PCA when the data may be corrupted by outliers. Recent work by Cand{\`e}s, Wright, Li, and Ma defined RPCA as a problem of decomposing a given data matrix into the sum of a low-rank matrix (true data) and a sparse matrix (outliers). The column space of the low-rank matrix then gives the PCA solution. This simple definition has lead to a large amount of interesting new work on provably correct, fast, and practical solutions to RPCA. More recently, the dynamic (time-varying) version of the RPCA problem has been studied and a series of provably correct, fast, and memory efficient tracking solutions have been proposed. Dynamic RPCA (or robust subspace tracking) is the problem of tracking data lying in a (slowly) changing subspace while being robust to sparse outliers. This article provides an exhaustive review of the last decade of literature on RPCA and its dynamic counterpart (robust subspace tracking), along with describing their theoretical guarantees, discussing the pros and cons of various approaches, and providing empirical comparisons of performance and speed. A brief overview of the (low-rank) matrix completion literature is also provided (the focus is on works not discussed in other recent reviews). This refers to the problem of completing a low-rank matrix when only a subset of its entries are observed. It can be interpreted as a simpler special case of RPCA in which the indices of the outlier corrupted entries are known.

==> PCA_outliers.tex <==

\pgfplotstableread[col sep = comma]{small_noise_twod.dat}\sninp
\pgfplotstableread[col sep = comma]{large_noise_twod.dat}\lninp

\pgfplotsset{every axis title/.style={text width=.5\textwidth, align=center, at={(.5, -0.2)}, below}}
\begin{figure*}[t!]
\begin{center}
\begin{tikzpicture}
    \begin{groupplot}[
        group style={
            group size=2 by 1,
            x descriptions at=edge bottom,
            y descriptions at=edge left,
        },
        % load the style created in the preamble
        %my stylecompare,
        height=5cm,
        width=.5\textwidth,
        %
        % define the axis limits for the plots ...
        xmin=-12,xmax=12,
        ymin=-20, ymax=30,
        % ... and enlarge them a bit (use the default value)
        %enlargelimits=false,
    ]
       \nextgroupplot[
       axis x line*=box,
		axis y line*=box,
            %my legend style compare,
            %ymode=log,
            %xlabel=$t$,
            title={(a) SVD on data corrupted by small noise finds the correct PC}
        ]
                \node [text width=1em,anchor=north west] at (rel axis cs: 0.45,-1.2)
                {\subcaption{\label{fig:small_noise}}};


	        \addplot[%
	        scatter=false,
	        only marks,
	        mark=o,
	        color=red,
	        on layer=background] table[x index = {0}, y index = {1}]{\sninp};
	
	            	        \addplot[black,
	        line width=3pt,
	        on layer=foreground] table[x index = {2}, y index = {3}]{\sninp};
	
	
        \nextgroupplot[
               axis x line*=box,
		axis y line*=box,
            %ymode=log,
            %xlabel=$t$,
            title={(b) SVD on outlier-corrupted data provides a wrong estimate of the PC}
        ]
        \node [text width=1em,anchor=north west] at (rel axis cs: 0.45,-1.2)
                {\subcaption{\label{fig:large_noise}}};

        \addplot[%
	        scatter=false,
	        only marks,
	        mark=o,
	        color=red,
	        on layer=main] 	
	        table[x index = {0}, y index = {1}]{\lninp};
	        \addplot[black,
	        line width=2pt,
	        on layer=main]
%	        ,
%	        mark=square,
%	        mark size=0.7pt]
	        table[x index = {2}, y index = {3}]{\lninp};
	
	    \end{groupplot}
\end{tikzpicture}
\end{center}
\caption{\small{(a) PCA in small noise: the SVD solution works. The black line is the estimated principal component computed using the observed data. %This clearly approximates the direction of largest variance of the data correctly.
(b) PCA in outliers: the SVD solution fails to correctly find the direction of largest variance of the true data. Instead its estimate is quite far from the true principal component.
}}
%For both cases, we generated data as $\l_i = 5 + 2x_i$, where $x_i$'s are $1000$ uniformly spaced points between $-10$ and $10$. In Fig. \ref{fig:small_noise} we generated the noise $z$ as independent samples from $z_i \overset{iid}{\sim} \mathcal{N}(0, 3)$ distribution. Note that the principal component, indicated by the black line is able to track the ``direction of largest variation'', or the first principal component accurately. However, in Fig. \ref{fig:large_noise} where we generated the same underlying data but the noise was generated as a mixture of Gaussians, such that $z_i \overset{iid}{\sim} 0.99 \mathcal{N}(0, 1) + 0.01 \mathcal{N}(0, 200)$. In this case, the principal component is visibly distorted.}}
\label{PCA_outliers}
\end{figure*}


==> all_grouse_guarantees.tex <==
\subsection{Dynamic MC or Subspace Tracking with missing data} \label{subtrack}
%The three well known algorithms for ST-missing are PAST, PETRELS and GROUSE \cite{past,past_conv,petrels,grouse,local_conv_grouse}. These and many others are described in detail in a review article on subspace \cite{chi_review}.
\color{red}
In the literature, there are three well-known algorithms for subspace tracking with missing data (equivalently, dynamic MC): PAST \cite{past,past_conv}, PETRELS \cite{petrels} and GROUSE \cite{grouse,local_conv_grouse, grouse_global, grouse_enh}. All are motivated by stochastic gradient descent to solve the PCA problem and the Oja algorithm.  These and many others are described in detail in a review article on subspace \cite{chi_review}. In this section, we briefly summarize the theoretical guarantees this problem: the only result for missing data is for GROUSE for the case of {\em single unknown subspace}. Moreover, the result is a {\em partial guarantee (result makes assumptions on intermediate algorithm estimates)}.




To our best knowledge, with the exception of \cite{grouse_global}, all the come with asymptotic and partial guarantees (make assumptions about intermediate algorithm estimates), and furthermore, {\em all} guarantees assume a single unknown subspace. We provide one sample guarantee here just in order to serve as a benchmark to compare the robust ST results.

%All guarantees assume a {\em single unknown} subspace and all guarantees are either asymptotic or are partial guarantees (make assumptions about intermediate algorithm estimates).
%PAST has a complete but asymptotic guarantee only when $r=1$ and there is no missing data, i.e., when $\yt = \lt + \vt$. It says the following \cite{past,past_conv}.
%\begin{theorem}
%Suppose the unknown subspace is fixed, denote it by $\P$. Assume it is an $r=1$ dimensional subspace. As long as initialization satisfies $R(0) > 0$, $w_{(0)}{}'\P \neq 0$, the output of PASTd converges to the true subspace $\P$ as $t \to \infty$.
%\end{theorem}

%The guarantee for PAST says the following
%\begin{theorem}
%Under mild conditions of initialization which say that the energy along the signal subspace is non-zero, and few assumptions on the intermediate algorithm estimates, the PAST algorithm converges to the global minimum asymptotically.
%\end{theorem}

%and uniformly at random
The guarantee for GROUSE says the following in the fully observed setting \cite{local_conv_grouse}. This is the setting when there is no missing data, i.e., $\yt =\lt + \vt$. Intuitively, this result tells us that in the fully observed setting, GROUSE is guaranteed to converge to a local minima of the optimization problem.
\begin{theorem}[GROUSE-full]
Suppose the unknown subspace is fixed, denote it by $\P$.
Let $\Phat_{(t)}$ denote the estimate of the subspace at time $t$. Let $\epsilon_t = \sum_{i=1}^r \sin^2\theta_i(\Phat_{(t)}, \P)$ where $\theta_i$ is the $i$-th principal angle. Assume that for each time $t$, $\epsilon_t \leq \bar{\epsilon} \in (0, 1/3)$. Let the entries of $\at$ be drawn independently  from a standard normal distribution. Then, the output of the algorithm satisfies
\begin{align*}
\mathbb{E}[\epsilon_{t+1} | \epsilon_t] \leq \left( 1 - \frac{1 - 3 \epsilon_t}{r} \right)\epsilon_t
\end{align*}
\end{theorem}
The above result is a partial guarantee. It requires assuming that $\epsilon_t$ is bounded below a constant less than $1/3$ at each time $t$ (but the guarantee only bounds the conditional expectation of $\epsilon_t$).


The latest guarantee for GROUSE \cite{grouse_global} provides the the following guarantees in the fully observed setting. This is a much stronger result than the previous result which says that GROUSE actually converges to the global minima in the fully observed setting. First, for simplicity we assume that there is no noise, i.e., $\yt = \lt$ and the goal is to recover $\P$.

\begin{theorem}[GROUSE-global-noiseless]
Suppose the unknown subspace is fixed, denote it by $\P$.
Let $\Phat_{(t)}$ denote the estimate of the subspace at time $t$. Let $\epsilon_t = \sum_{i=1}^r \sin^2\theta_i(\Phat_{(t)}, \P)$ where $\theta_i$ is the $i$-th principal angle and $\zeta_t = \prod_{i=1}^r \cos^2\theta_i(\Phat_{(t)}, \P_t)$. Assume that the initial estimate, $\Phat_{(0)}$ is obtained by a random initialization, i.e., it is obtained by orthonormalizing a $n \times r$ i.i.d. standard normal matrix. Then, for any $\epsilon_\ast > 0$ (desired accuracy) and any $\delta, \delta{}' >0$ (desired failure probabilities), after
\begin{align*}
T= K_1 + K_2 = \left(\frac{r^3}{\rho{}'} + r \right)\mu_0 \log n + 2r\log\left( \frac{1}{\epsilon_\ast \rho}\right) \\
\end{align*}
iterations, with probability at least $1 - \delta - \delta{}'$, GROUSE satisfies $\epsilon_T \leq \epsilon_\ast$. Here, $\mu = 1 + \frac{\log((1 - \delta{}')/C + r \log(e/r)}{r\log n}$ for a constant $C \approx 1$.
\end{theorem}

Now, we consider the case when there is additional white Gaussian noise, i.e., $\yt = \lt + \wt$ such that $\mathbb{E}[\wt] = \bm{0}$ and $\mathbb{E}[\|\wt\|^2/\|\lt\|^2 | \lt]  \leq \sigma^2$. Then, \cite{grouse_global} provides the following two guarantee, in terms of two error metrics respectively, for {\em one iteration} of GROUSE
\begin{theorem}[GROUSE-global-noisy-1]
Suppose the unknown subspace is fixed, denote it by $\P$.
Let $\Phat_{(t)}$ denote the estimate of the subspace at time $t$. Let $\zeta_t = \prod_{i=1}^r \cos^2\theta_i(\Phat_{(t)}, \P_t)$. Assume that the initial estimate, $\Phat_{(0)}$ is obtained by a random initialization, i.e., it is obtained by orthonormalizing a $n \times r$ i.i.d. standard normal matrix. Then, for any the following improvement is obtained in expectation
\begin{align*}
\mathbb{E}\left[\zeta_{t+1} \big| \Phat_{(t)} \right] \geq \left( 1 + \frac{\beta_0}{(1 - \zeta_t)/r + \sigma^2}\left(\frac{1 - \zeta_t}{r}\right)^2 \right)\zeta_t
\end{align*}
where $\beta_0 = \frac{1}{1 + r\sigma^2/n}$.
\end{theorem}

\begin{theorem}[GROUSE-global-noisy-2]
Suppose the unknown subspace is fixed, denote it by $\P$.
Let $\Phat_{(t)}$ denote the estimate of the subspace at time $t$. Let $\epsilon_t = \sum_{i=1}^r \sin^2\theta_i(\Phat_{(t)}, \P)$. Assume that the initial estimate, $\Phat_{(0)}$ is obtained by a random initialization, i.e., it is obtained by orthonormalizing a $n \times r$ i.i.d. standard normal matrix. Then, for any the following improvement is obtained in expectation
\begin{align*}
\mathbb{E}\left[\epsilon_{t+1} \big| \Phat_{(t)} \right] &\leq \\
&\left( 1 - \frac{\beta_0}{r}\left(\cos^2\theta_1(\Phat_{(t)}, \P) - \frac{\beta_1\sigma^2}{\epsilon_t/r + \beta_1\sigma^2}\right)\right)\epsilon_t
\end{align*}
where $\beta_0 = \frac{1}{1 + r\sigma^2/n}$, $\beta_1 = 1 - r/n$ and $\theta_1(\Phat_{(t)}, \P_t)$ is the largest principal angle between the arguments.
\end{theorem}

\color{black}

The guarantee for GROUSE \cite{local_conv_grouse} says the following in the partially observed setting. %Recall that $\P$ is $\mu$-incoherent, and $\epsilon_t$ is defined as the square of the chordal distance between the subspace estimate $\Phat_{(t)}$ and the true subspace $\P$.
%We also need the following generalization of incoherence for a vector
%\begin{definition}
%For a vector $\bm{x} \in \mathbb{R}^n$ define
%\begin{align*}
%\mu(\bm{x}) :=  \frac{n \norm{\bm{x}}^2_{\infty}}{\norm{\bm{x}}^2_{2}}
%\end{align*}
%\end{definition}

% and uniformly at random
\begin{theorem}[GROUSE-partial]
Suppose the unknown subspace is fixed, denote it by $\P$. Assume it is $\mu$-incoherent and  the following hold
\begin{enumerate}
\item Let the entries of $\at$ be drawn independently from a standard Normal distribution, i.e., $(\at)_i \overset{i.i.d.}{\sim} \mathcal{N}(0, 1)$.
\item The set of observed entries at time $t$ is $\Omega_t$. Assume that the number of entries observed at each time satisfies $|\Omega_t| \geq q$ where $q \geq (64/3)\cdot r \log^2 n \mu \log(20r)$.
\item $\epsilon_t$ satisfies
$
\epsilon_t \leq \min\left\{\frac{r \mu}{16n}, \frac{q^2}{128 n^2  r} \right\}
$
\item the residual at each time, $\bm{r}_t := \lt - \Phat_{(t)}\Phat_{(t)}' \lt$ satisfies
\begin{align*}
\mu(\bm{r}_t) \leq \min\bigg\{ \log n \left[\frac{0.045}{\log 10} C_1 r \mu \log(20 r)\right]^{0.5}, \\
 \log^2 n \frac{0.05}{8 \log 10} C_1 \log(20 r) \bigg\}
\end{align*}
with probability at least $1 - \bar{\delta}$ where $\bar{\delta} \leq 0.6$.
\end{enumerate}
Then, the output of the algorithm satisfies
\begin{align*}
\mathbb{E}[\epsilon_{t+1} | \epsilon_t] \leq \epsilon_t -.32(.6 - \bar{\delta}) \frac{q}{nr}\epsilon_t + 55 \sqrt{\frac{n}{q}} \epsilon_t^{1.5}
\end{align*}
\end{theorem}
The above result is also a partial guarantee. Moreover it is hard to parse since it needs many assumptions on $\epsilon_t$. It also needs a denseness assumption on the residual at each time $\bm{r}_t := \lt - \Phat_{(t)}\Phat_{(t)}' \lt$. This is similar to the denseness assumption on the currently un-updated subspace needed by the first (partial) guarantee for ReProCS from \cite{rrpcp_perf}.
%Also, the theorem conclusion is not easy to interpret.

